Not-so-Cleansing Recessions

Recessions are periods in which the least productive firms in the economy exit, and as the economy recovers, they are replaced by new and more productive entrants. These cleansing effects improve the average firm productivity. At the same time, recessions induce a loss of varieties. In an economy with Homothetic Single Aggregator technology, we show that their long-run welfare effects trade off these two forces. This trade-off is governed by love-of-variety and the elasticity of substitution in aggregate production. If industry output is aggregated using the standard CES aggregator, recessions do not improve long-run GDP or welfare. If the economy features more love-of-variety than CES, the social planner optimally subsidizes economic activity both in steady state and even more so in recessions to avoid firm exit. We use the model and quasi-exogenous variation in demand to estimate love-of-variety. We find it to be significantly higher than implied by CES aggregation, suggesting that even the long-run effects of recessions are negative. Finally, we quantitatively characterize the optimal policy response both along the transition and in the steady state.

==> figures/main_result_inst.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}\begin{tabular}{l*{2}{c}} \hline\hline & \multicolumn{1}{c}{{First Stage}} & Second Stage \\ \midrule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{$\Delta\log\mathcal{I}^r_{it} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{it}$}\\
\hline
 $  \eta_{it}^r $   &       0.133\sym{***}&                     \\
                    &   (0.00640)         &                     \\
[1em]
$\Delta \log P^r_{it}$&      -0.159\sym{***}&      0.0905\sym{***}\\
                    &   (0.00944)         &    (0.0108)         \\
[1em]
$\Delta \log \mathcal{Z}^r_{it}$&    -0.00442\sym{*}  &   -0.000852         \\
                    &   (0.00247)         &   (0.00447)         \\
[1em]
$\Delta\log\mathcal{I}^r_{it} $&                     &       1.512\sym{***}\\
                    &                     &    (0.0728)         \\
\hline
Country-Industry FE &         Yes         &         Yes         \\
F-Stat              &         431         &         151         \\
N                   &       21776         &       21776         \\
 $ R^2 $            &       0.192         &        0.486         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors are clustered at the producing industry $\times$ country level.}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_1.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}\begin{tabular}{l*{2}{c}} \hline\hline & \multicolumn{2}{c}{(A)} \\ \midrule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &      0.0854\sym{***}&                     \\
                    &    (0.0215)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0941\sym{***}&                     \\
                    &    (0.0231)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.512\sym{***}\\
                    &                     &     (0.191)         \\
\hline
$ P(q \leq q^{CES})) $&                     &         .07         \\
Year FE             &         Yes         &         Yes         \\
Industry FE         &         Yes         &         Yes         \\
F-Stat              &          22         &          63         \\
N                   &       10067         &       10067         \\
$ R^2 $             &      0.0315         &      0.0860         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Robust Standard Errors (HC1).}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_1112.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(E)} & \multicolumn{2}{c}{(F)} \\
                    &\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
                &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &       0.129\sym{***}&                     &       0.119\sym{***}&                     \\
                    &    (0.0213)         &                     &    (0.0204)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.377\sym{***}&                     &       1.668\sym{***}\\
                    &                     &    (0.0987)         &                     &     (0.101)         \\
\hline
                 &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &       0.105\sym{***}&                     &       0.101\sym{***}&                     \\
                    &    (0.0167)         &                     &    (0.0160)         &                     \\
$\Delta \log L^{d,r}_{i,t} $&                     &       1.689\sym{***}&                     &       1.970\sym{***}\\
                    &                     &     (0.127)         &                     &     (0.125)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat eq.(1)       &          36         &         166         &          33         &         202         \\
F-Stat eq.(2)       &          39         &          98         &          38         &         124         \\
N                   &       15028         &       15028         &       15028         &       15028         \\
$ R^2 $ eq.(1)      &     0.00664         &       0.131         &      0.0271         &       0.165         \\
$ R^2 $ eq.(2)      &     0.00715         &      0.0412         &      0.0323         &      0.0788         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors are clustered at the producing industry $\times$ country level.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_12.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c}{(B)} \\ & \multicolumn{1}{c}{First Stage} & \multicolumn{1}{c}{Second Stage} & \multicolumn{1}{c}{First Stage} & \multicolumn{1}{c}{Second Stage} \\ \midrule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &       0.126\sym{***}&                     &       0.116\sym{***}&                     \\
                    &    (0.0215)         &                     &    (0.0207)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.436\sym{***}&                     &       1.737\sym{***}\\
                    &                     &     (0.210)         &                     &     (0.267)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          33         &          46         &          31         &          42         \\
N                   &       15031         &       15030         &       15031         &       15030         \\
$ R^2 $             &     0.00610         &       0.263         &      0.0264         &       0.292         \\
\hline\hline
\end{tabular}
}


==> figures/model_1234.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c c c| c c c c} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c|}{(B)} & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c|}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &       0.124\sym{***}&                     &       0.114\sym{***}&                     &       0.108\sym{***}&                     &       0.104\sym{***}&                     \\
                    &    (0.0215)         &                     &    (0.0206)         &                     &    (0.0175)         &                     &    (0.0170)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.441\sym{***}&                     &       1.745\sym{***}&                     &                     &                     &                     \\
                    &                     &     (0.212)         &                     &     (0.269)         &                     &                     &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &                     &                     &       1.663\sym{***}&                     &       1.919\sym{***}\\
                    &                     &                     &                     &                     &                     &     (0.263)         &                     &     (0.304)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          33         &          46         &          30         &          41         &          38         &          40         &          37         &          39         \\
N                   &       15029         &       15029         &       15029         &       15029         &       15048         &       15048         &       15048         &       15048         \\
$ R^2 $             &     0.00615         &       0.262         &      0.0264         &       0.291         &     0.00725         &      0.0840         &      0.0317         &       0.116         \\
\hline\hline
\end{tabular}
}


==> figures/model_1234_v2.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c c c| c c c c} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c|}{(B)} & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &       0.124\sym{***}&                     &       0.114\sym{***}&                     &       0.108\sym{***}&                     &       0.104\sym{***}&                     \\
                    &    (0.0215)         &                     &    (0.0206)         &                     &    (0.0175)         &                     &    (0.0170)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.441\sym{***}&                     &       1.745\sym{***}&                     &                     &                     &                     \\
                    &                     &     (0.212)         &                     &     (0.269)         &                     &                     &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &                     &                     &       1.663\sym{***}&                     &       1.919\sym{***}\\
                    &                     &                     &                     &                     &                     &     (0.263)         &                     &     (0.304)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          33         &          46         &          30         &          41         &          38         &          40         &          37         &          39         \\
N                   &       15029         &       15029         &       15029         &       15029         &       15048         &       15048         &       15048         &       15048         \\
$ R^2 $             &     0.00615         &       0.262         &      0.0264         &       0.291         &     0.00725         &      0.0840         &      0.0317         &       0.116         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize }\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> figures/model_13141516.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c c c| c c c c} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c|}{(B)} & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c|}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t-1}^{+,r} $ &       0.118\sym{***}&                     &       0.104\sym{***}&                     &       0.120\sym{***}&                     &       0.112\sym{***}&                     \\
                    &    (0.0224)         &                     &    (0.0215)         &                     &    (0.0165)         &                     &    (0.0167)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.435\sym{***}&                     &       1.680\sym{***}&                     &                     &                     &                     \\
                    &                     &     (0.230)         &                     &     (0.294)         &                     &                     &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &                     &                     &       1.420\sym{***}&                     &       1.568\sym{***}\\
                    &                     &                     &                     &                     &                     &     (0.182)         &                     &     (0.217)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          27         &          38         &          23         &          32         &          52         &          61         &          45         &          52         \\
N                   &       15507         &       15507         &       15507         &       15507         &       15526         &       15526         &       15526         &       15526         \\
$ R^2 $             &     0.00878         &       0.336         &      0.0254         &       0.353         &      0.0112         &       0.146         &      0.0353         &       0.166         \\
\hline\hline
\end{tabular}
}


==> figures/model_1718.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(E)} & \multicolumn{2}{c}{(F)} \\ 
                    &\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
                &                     &                     &                     &                     \\
 $ \eta_{i,t-1}^{+,r} $ &       0.117\sym{***}&                     &       0.104\sym{***}&                     \\
                    &    (0.0224)         &                     &    (0.0215)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.438\sym{***}&                     &       1.684\sym{***}\\
                    &                     &     (0.106)         &                     &     (0.118)         \\
\hline
                 &                     &                     &                     &                     \\
 $ \eta_{i,t-1}^{+,r} $ &       0.118\sym{***}&                     &       0.111\sym{***}&                     \\
                    &    (0.0164)         &                     &    (0.0165)         &                     \\
$\Delta \log L^{d,r}_{i,t} $&                     &       1.424\sym{***}&                     &       1.576\sym{***}\\
                    &                     &     (0.112)         &                     &     (0.117)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat eq.(1)       &          27         &         186         &          23         &         201         \\
F-Stat eq.(2)       &          52         &          94         &          44         &         101         \\
N                   &       15505         &       15505         &       15505         &       15505         \\
$ R^2 $ eq.(1)      &     0.00877         &       0.208         &      0.0254         &       0.228         \\
$ R^2 $ eq.(2)      &      0.0111         &       0.109         &      0.0352         &       0.133         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors are clustered at the producing industry $\times$ country level.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_19202122.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c c c| c c c c} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c|}{(B)} & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c|}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &      0.0928\sym{***}&                     &      0.0854\sym{***}&                     &       0.105\sym{***}&                     &       0.103\sym{***}&                     \\
                    &    (0.0229)         &                     &    (0.0223)         &                     &    (0.0211)         &                     &    (0.0207)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0981\sym{***}&                     &      0.0941\sym{***}&                     &      0.0659\sym{***}&                     &      0.0646\sym{**} &                     \\
                    &    (0.0242)         &                     &    (0.0240)         &                     &    (0.0199)         &                     &    (0.0204)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.246\sym{***}&                     &       1.512\sym{***}&                     &                     &                     &                     \\
                    &                     &     (0.183)         &                     &     (0.229)         &                     &                     &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &                     &                     &       1.409\sym{***}&                     &       1.634\sym{***}\\
                    &                     &                     &                     &                     &                     &     (0.204)         &                     &     (0.237)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          16         &          46         &          15         &          43         &          22         &          47         &          21         &          47         \\
N                   &       10068         &       10068         &       10067         &       10067         &       10084         &       10084         &       10083         &       10083         \\
$ R^2 $             &     0.00943         &       0.278         &      0.0315         &       0.315         &      0.0110         &      0.0810         &      0.0413         &       0.122         \\
\hline\hline
\end{tabular}
}


==> figures/model_2324.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(E)} & \multicolumn{2}{c}{(F)} \\ 
                    &\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
                &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &      0.0928\sym{***}&                     &      0.0853\sym{***}&                     \\
                    &    (0.0228)         &                     &    (0.0222)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0972\sym{***}&                     &      0.0932\sym{***}&                     \\
                    &    (0.0240)         &                     &    (0.0238)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.169\sym{***}&                     &       1.396\sym{***}\\
                    &                     &    (0.0956)         &                     &    (0.0936)         \\
\hline
                 &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &       0.104\sym{***}&                     &       0.101\sym{***}&                     \\
                    &    (0.0211)         &                     &    (0.0206)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0650\sym{***}&                     &      0.0634\sym{***}&                     \\
                    &    (0.0198)         &                     &    (0.0202)         &                     \\
$\Delta \log L^{d,r}_{i,t} $&                     &       1.286\sym{***}&                     &       1.471\sym{***}\\
                    &                     &     (0.111)         &                     &     (0.104)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat eq.(1)       &          16         &         130         &          15         &         161         \\
F-Stat eq.(2)       &          23         &          75         &          22         &          97         \\
N                   &       10067         &       10067         &       10067         &       10067         \\
$ R^2 $ eq.(1)      &     0.00942         &       0.143         &      0.0315         &       0.187         \\
$ R^2 $ eq.(2)      &      0.0108         &      0.0465         &      0.0410         &      0.0929         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors are clustered at the producing industry $\times$ country level.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_34.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\ & \multicolumn{1}{c}{First Stage} & \multicolumn{1}{c}{Second Stage} & \multicolumn{1}{c}{First Stage} & \multicolumn{1}{c}{Second Stage} \\ \midrule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &       0.109\sym{***}&                     &       0.105\sym{***}&                     \\
                    &    (0.0175)         &                     &    (0.0170)         &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &       1.665\sym{***}&                     &       1.920\sym{***}\\
                    &                     &     (0.262)         &                     &     (0.304)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          38         &          40         &          38         &          39         \\
N                   &       15049         &       15049         &       15049         &       15049         \\
$ R^2 $             &     0.00726         &      0.0840         &      0.0318         &       0.116         \\
\hline\hline
\end{tabular}
}


==> figures/model_56.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l*{4}{c}} \hline\hline & \multicolumn{2}{c}{(E)} & \multicolumn{2}{c}{(F)} \\ 
                    &\multicolumn{1}{c}{$\Delta \log {X}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log X^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
                &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &       0.124\sym{***}&                     &       0.114\sym{***}&                     \\
                    &    (0.0215)         &                     &    (0.0206)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.443\sym{***}&                     &       1.748\sym{***}\\
                    &                     &     (0.105)         &                     &     (0.108)         \\
\hline
                &                     &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &       0.107\sym{***}&                     &       0.103\sym{***}&                     \\
                    &    (0.0175)         &                     &    (0.0168)         &                     \\
                 &                     &                     &                     &                     \\
$\Delta \log L^{d,r}_{i,t} $&                     &       1.677\sym{***}&                     &       1.940\sym{***}\\
                    &                     &     (0.128)         &                     &     (0.126)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         \\
F-Stat eq.(1)       &          33         &         161         &          30         &         194         \\
F-Stat eq.(2)       &          37         &          95         &          36         &         119         \\
N                   &       15028         &       15028         &       15028         &       15028         \\
$ R^2 $ eq.(1)      &     0.00615         &       0.130         &      0.0265         &       0.163         \\
$ R^2 $ eq.(2)      &     0.00714         &      0.0406         &      0.0316         &      0.0772         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors are clustered at the producing industry $\times$ country level.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_78910.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c c c| c c c c} \hline\hline & \multicolumn{2}{c}{(A)} & \multicolumn{2}{c|}{(B)} & \multicolumn{2}{c}{(C)} & \multicolumn{2}{c}{(D)} \\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c|}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &       0.129\sym{***}&                     &       0.119\sym{***}&                     &       0.107\sym{***}&                     &       0.103\sym{***}&                     \\
                    &    (0.0213)         &                     &    (0.0204)         &                     &    (0.0168)         &                     &    (0.0161)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.376\sym{***}&                     &       1.665\sym{***}&                     &                     &                     &                     \\
                    &                     &     (0.194)         &                     &     (0.244)         &                     &                     &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &                     &                     &       1.675\sym{***}&                     &       1.947\sym{***}\\
                    &                     &                     &                     &                     &                     &     (0.257)         &                     &     (0.299)         \\
\hline
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &          No         &          No         &         Yes         &         Yes         &          No         &          No         &         Yes         &         Yes         \\
F-Stat              &          36         &          50         &          34         &          46         &          40         &          42         &          40         &          42         \\
N                   &       15029         &       15029         &       15029         &       15029         &       15048         &       15048         &       15048         &       15048         \\
$ R^2 $             &     0.00664         &       0.264         &      0.0270         &       0.293         &     0.00726         &      0.0850         &      0.0324         &       0.118         \\
\hline\hline
\end{tabular}
}


==> figures/model_AB.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi} \begin{tabular}{l c c | c c} \hline\hline & \multicolumn{2}{c|}{(A)} & \multicolumn{2}{c}{(B)} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c|}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c|}{$\Delta \log Y^r_{i,t}$}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
 $ \eta_{i,t}^{+,r} $ &      0.0854\sym{***}&                     &       0.103\sym{***}&                     \\
                    &    (0.0215)         &                     &    (0.0204)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0941\sym{***}&                     &      0.0646\sym{***}&                     \\
                    &    (0.0231)         &                     &    (0.0204)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &       1.512\sym{***}&                     &                     \\
                    &                     &     (0.191)         &                     &                     \\
[1em]
$\Delta \log L^{d,r}_{i,t} $&                     &                     &                     &       1.634\sym{***}\\
                    &                     &                     &                     &     (0.245)         \\
\hline
$ P(q \leq q^{CES}) $&                     &         .07         &                     &        .049         \\
Year FE             &         Yes         &         Yes         &         Yes         &         Yes         \\
Industry FE         &         Yes         &         Yes         &         Yes         &         Yes         \\
F-Stat              &          22         &          63         &          23         &          45         \\
N                   &       10067         &       10067         &       10083         &       10083         \\
$ R^2 $             &      0.0315         &      0.0860         &      0.0413         &      0.0880         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Robust Standard Errors (HC1).}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/model_C.tex <==
{\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}\begin{tabular}{l*{3}{c}} \hline\hline & \multicolumn{3}{c}{(C)} \\ \midrule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{$\Delta \log \mathcal{I}^r_{i,t} $}&\multicolumn{1}{c}{$\Delta \log L^{d,r}_{i,t} $}&\multicolumn{1}{c}{$\Delta \log Y^r_{i,t}$}\\
\hline
                &                     &                     &                     \\
 $ \eta_{i,t}^{+,r} $ &      0.0853\sym{***}&       0.101\sym{***}&                     \\
                    &    (0.0215)         &    (0.0204)         &                     \\
[1em]
 $ \eta_{i,t-1}^{+,r} $ &      0.0932\sym{***}&      0.0634\sym{***}&                     \\
                    &    (0.0231)         &    (0.0204)         &                     \\
[1em]
$\Delta \log \mathcal{I}^r_{i,t} $&                     &                     &       1.568\sym{***}\\
                    &                     &                     &     (0.151)         \\
$\Delta \log L^{d,r}_{i,t} $&                     &                     &       1.568\sym{***}\\
                    &                     &                     &     (0.151)         \\
\hline
$ P(q \leq q^{CES}) $&                     &                     &        .013         \\
Year FE             &                     &         Yes         &         Yes         \\
Industry FE         &                     &         Yes         &         Yes         \\
F-Stat eq.(1)       &          22         &                     &        2843         \\
F-Stat eq.(2)       &                     &          22         &         131         \\
N                   &       10066         &       10066         &       10067         \\
$ R^2 $ eq.(1)      &        .032         &                     &      0.0870         \\
$ R^2 $ eq.(2)      &                     &        .041         &      0.0880         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Robust Standard Errors (HC1).}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> figures/profit_sigma_qces_table_es.tex <==
\begin{table}[htp]
\centering
\small
\caption{Distribution of Profit Rate, $ \sigma $, and $ q^{CES} $ in Spain}
\label{tab:profit_sigma_qces_spain}
\begin{tabular}{l c c c}
\hline\hline
Percentiles & | \hspace{0.1cm} \textbf{Profit Rate} \hspace{0.1cm} | & $ \boldsymbol{\sigma} $ & | \hspace{0.2cm} $ \mathbf{q^{CES}} $ \\
\hline
1 & -13.1\% & -29.6 & -0.12 \\
5 & 3.0\% & 1.5 & 0.03 \\
10 & 6.6\% & 2.0 & 0.07 \\
25 & 11.9\% & 3.1 & 0.14 \\
50 & 19.4\% & 4.9 & 0.24\\
75 & 30.4\% & 7.7 & 0.44 \\
90 & 44.6\% & 12.4 & 0.81 \\
95 & 54.2\% & 17.4 & 1.18 \\
99 & 70.1\% & 47.1 & 2.35 \\
\hline\hline
\end{tabular}
\end{table}

==> figures/summary_stats_q_CES_ind.tex <==
\begin{table}[H]
\centering
\small
\caption{Descriptive Statistics of $ q^{CES} $ across Industries}
\label{tab:sigma_est}
\begin{tabular}{l c c| l c }
\hline\hline
\multicolumn{1}{c|}{\textbf{Percentiles}}& $q^{CES}$ & \textbf{Implied Profit Rate}& \multicolumn{2}{c}{\textbf{Moments $q^{CES}$}} \\
\midrule
1 & .05 & 4.8\%& Mean & .29 \\
5 & .07 &6.5\%& Variance & .05 \\
10 & .09 &8.3\%& Skewness & 2.55 \\
25 & .15 &13\%& Kurtosis & 11.63 \\
50 & .23 &18.7\%&  &  \\
75 & .37 &27\%&  &  \\
90 & .49 &32.9\%&  &  \\
95 & .73 &42.2\%&  &  \\
99 & 1.37 &57.9\%&  &  \\
\hline\hline
\end{tabular}
\end{table}

==> figures/summary_stats_q_CES_ind_final.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Distribution of Profit Rate, $ \sigma $, and $ q^{CES} $ across Industries}
\label{tab:profit_sigma_qces}
\begin{tabular}{l c c c}
\hline\hline
Percentiles & | \hspace{0.1cm} \textbf{Profit Rate} \hspace{0.1cm} | & $ \boldsymbol{\sigma} $ & | \hspace{0.2cm} $ \mathbf{q^{CES}} $ \\
\hline
1 & 0.0\% & 1.7 & 0.05 \\
5 & 6.2\% & 2.4 & 0.07 \\
10 & 7.6\% & 3.1 & 0.09 \\
25 & 12.7\% & 3.7 & 0.15 \\
\rowcolor{lightgray} 50 & 18.7\% & 5.3 & 0.23 \\
75 & 26.8\% & 7.5 & 0.37 \\
90 & 32.8\% & 12.4 & 0.49 \\
95 & 42.1\% & 15.3 & 0.73 \\
99 & 57.9\% & 22.6 & 1.37 \\
\hline\hline
\end{tabular}
\end{table}

% \begin{table}[H]
% \centering
% \small
% \caption{Distribution of Profit Rate, $ \sigma $, and $ q^{CES} $ across Industries}
% \label{tab:profit_sigma_qces}
% \begin{tabular}{l c c c c c c}
% \toprule
%  & \multicolumn{3}{c}{\textit{A. WIOD}} & \multicolumn{3}{c}{\textit{B. Spain}} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% Percentiles & \textbf{Profit Rate} & $ \boldsymbol{\sigma} $ & $ \mathbf{q^{CES}} $
%             & \textbf{Profit Rate} & $ \boldsymbol{\sigma} $ & $ \mathbf{q^{CES}} $ \\
% \midrule
% 1  & 0.0\%  & 1.7  & 0.05 & 0.0\%  & 1.7  & 0.05 \\
% 5  & 6.2\%  & 2.4  & 0.07 & 6.2\%  & 2.4  & 0.07 \\
% 10 & 7.6\%  & 3.1  & 0.09 & 7.6\%  & 3.1  & 0.09 \\
% 25 & 12.7\% & 3.7  & 0.15 & 12.7\% & 3.7  & 0.15 \\
% \rowcolor{lightgray} 50 & 18.7\% & 5.3  & 0.23 & 18.7\% & 5.3  & 0.23 \\
% 75 & 26.8\% & 7.5  & 0.37 & 26.8\% & 7.5  & 0.37 \\
% 90 & 32.8\% & 12.4 & 0.49 & 32.8\% & 12.4 & 0.49 \\
% 95 & 42.1\% & 15.3 & 0.73 & 42.1\% & 15.3 & 0.73 \\
% 99 & 57.9\% & 22.6 & 1.37 & 57.9\% & 22.6 & 1.37 \\
% \bottomrule
% \end{tabular}
% \end{table}


==> figures/summary_stats_q_CES_ind_pt1.tex <==
\begin{table}[H]
\centering
\small
\caption{Percentile Summary Statistics}
\label{tab:percentiles}
\begin{tabular}{l c}
\hline\hline
 & \textbf{Percentiles} \\
\midrule
1 & .05 \\
5 & .07 \\
10 & .09 \\
25 & .15 \\
50 & .23 \\
75 & .37 \\
90 & .49 \\
95 & .73 \\
99 & 1.37 \\
\hline\hline
\end{tabular}
\end{table}


==> figures/summary_stats_q_CES_ind_pt2.tex <==
\begin{table}[H]
\centering
\small
\caption{Moment Statistics}
\label{tab:moments}
\begin{tabular}{l c}
\hline\hline
 & \textbf{Moments} \\
\midrule
Mean & .29 \\
Variance & .05 \\
Skewness & 2.55 \\
Kurtosis & 11.63 \\
\hline\hline
\end{tabular}
\end{table}


==> figures/summary_stats_q_CES_ind_v1.tex <==
\begin{table}[H]
\centering
\small
\caption{q CES v1 Summary Statistics}
\label{tab:summary}
\begin{tabular}{l c}
\hline\hline
\textbf{Statistic} & \textbf{Value} \\
\midrule
Percentile 1 & .05 \\
Percentile 5 & .08 \\
Percentile 10 & .1 \\
Percentile 25 & .17 \\
Median (50) & .25 \\
Percentile 75 & .37 \\
Percentile 90 & .65 \\
Percentile 95 & .76 \\
Percentile 99 & 1.57 \\
Mean & .32 \\
Standard Deviation & .27 \\
Minimum & .05 \\
Maximum & 1.57 \\
Skewness & 2.69 \\
Kurtosis & 11.85 \\
\hline\hline
\end{tabular}
\end{table}


==> figures/summary_stats_q_CES_ind_v2.tex <==
\begin{table}[H]
\centering
\small
\caption{q CES v2 Summary Statistics}
\label{tab:summary}
\begin{tabular}{l c}
\hline\hline
\textbf{Statistic} & \textbf{Value} \\
\midrule
Percentile 1 & .05 \\
Percentile 5 & .1 \\
Percentile 10 & .12 \\
Percentile 25 & .23 \\
Median (50) & .35 \\
Percentile 75 & .55 \\
Percentile 90 & .77 \\
Percentile 95 & .97 \\
Percentile 99 & 1.17 \\
Mean & .42 \\
Standard Deviation & .26 \\
Minimum & 0 \\
Maximum & 1.17 \\
Skewness & 1.01 \\
Kurtosis & 3.62 \\
\hline\hline
\end{tabular}
\end{table}

